A Survey on Physarum Polycephalum Intelligent Foraging Behaviour and Bio-Inspired Applications

In recent years, research on Physarum polycephalum has become more popular after Nakagaki et al. (2000) performed their famous experiment showing that Physarum was able to find the shortest route through a maze. Subsequent researches have confirmed the ability of Physarum-inspired algorithms to solve a wide range of NP-hard problems. In contrast to previous reviews that either focus on biological aspects or bio-inspired applications, here we present a comprehensive review that highlights recent Physarum polycephalum biological aspects, mathematical models, and Physarum bio-inspired algorithms and their applications. The novelty of this review stems from our exploration of Physarum intelligent behaviour in competition settings. Further, we have presented our new model to simulate Physarum in competition, where multiple Physarum interact with each other and with their environments. The bio-inspired Physarum in competition algorithms proved to have great potentials for future research.

==> Algorithms/DMOO/PCO.tex <==
\begin{algorithm}
	\caption{Physarum-Inspired Competition Algorithm}
    \label{alg:DMOO/PCA}
	\BlankLine
    %\SetKwInOut{Input}{Input}
    %\SetKwInOut{Output}{Output}
    
    %\Input{
    %    $np$ (Total Number of Physarum)\newline
	%    $init\_pm$ (Initial Physarum Mass)
	%}
    %\Output{$GPF$ (Global Pareto front)}
    %\BlankLine
    %\tcc{Multiline comment}
    %\tcp{Initialize empty global Pareto front}
    $GPF = \{\}$ \tcp*{Initialize empty global Pareto front}
    
    \tcc{Initialize Physarum (solutions) $\{S = P_1, P_2,~\dots\ , P_{np}\}$} 
    \ForEach{Physarum $(P_{i})$}{ \label{alg:DMOO/Init_Physraum}
    
        $P_{i}.mass \gets init\_pm$ \tcp{Initialize Physarum mass}
      
        %$p.id \gets NEW\_ID$
      
        $P_{i}.lpf \gets \{\}$ \tcp{Initialize empty local Pareto front for Physarum}
      
        Randomly place Physarum (position vector) $P_{i}$ in the search space using either Monto Carlo or Latin Hypercube sampling techniques.
    }
    
    $current\text{-}iter = 0$
    
    \While{$current\text{-}iter < max\text{-}iter$} {
        
        \ForEach{Physarum $(P_{i})$}{%
            
            Add Physarum $P_{i}$ (solution) to it's $LPF$ (If not dominated by other solutions in Physarum $LPF$)
            
            %\ForEach{Objective Function  $f_i \in F$}{%
            %    Keep track of each Objective Function $f_i$ Minimum Value ($f_i\_Min$) and Maximum Value ($f_i\_Max$)
            %}
            %\newline
            
            \tcp{Initialize Physarum Neighbourhood}
            \ForEach{Physarum $P_{k}$ in Physarum $P_{i}$ Neighbourhood \tcp*{Definition \ref{equ:DMOO/Physarum_Neighbourhood}}}{
                \If{$P\_AA_{(P_{i}) \to (P_{k})} = 1$ \tcp*{Equation \ref{equ:DMOO/phy_aa}} }{
                    Add a new Physarum $(P_{k})$ to the search space with initial mass $0$
                    
                    %$new\_p.mass \gets 0$
                    
                    %$new\_p.id \gets p.id$
                    
                    %$np = np + 1$ \tcp{Increase number of Physarum (Solutions)}
                }
            }
        }
        \ForEach{Physarum $(P_{i})$}{%\ForEach{Physarum $p^n \in P : n=1,2, ..., np$}
            Diffuse $P^{t}_{i}$ to the neighbouring cells \tcp*{Equation \ref{equ:DMOO/phy_diff}}
        }
        \If{USING RESTART PROCEDURE}{ \label{alg:DMOO/Restart_Procedure}
            \If{$iteration~\%~restart\text{-}iteration = 0$}{
                %Keep the old global Pareto front
                
                Compute new $GPF$ from each Physarum $LPF$.
                
                %Subtract the old global Pareto front from the new global Pareto front
                
                Clear old Physarum (Solutions) and create others from this new $GPF$ (As in line \ref{alg:DMOO/Init_Physraum})
            }
        }
        $current\text{-}iter = current\text{-}iter + 1$
    }
    Compute $GPF$ from each Physarum $LPF$.% (Does this need more clarification) 
\end{algorithm}

==> Equations/DMOO/DMOO_Problem_DEF.tex <==
\begin{equation}
\label{equ:DMOO/DMOO_Problem_Def}
\begin{aligned}
& \textit{minimise}   
& & F(X) = (f_1(X), \ldots , f_m(X)), \{F : X \rightarrow R^m, m \geq 2\} \\
& \textit{subject to}
& & G(X) = (g_1(X), \ldots , g_k(X)), \{G : X \rightarrow R^k, G_k(X) \geq 0, k \geq 0\}\\
&
& & H(X) = (h_1(X), \ldots , h_l(X)), \{H : X \rightarrow R^l, H_l(X) = 0, l \geq 0\}\\
& \textit{and}
& & X = (x_1, \ldots , x_n), \{X \subset Z^n\}\\
\end{aligned}
\end{equation}
In the above equation,
$X$ is an n-dimensional decision variable (vector) from a discrete (Integer) space.
$F(X)$ is an objective vector composed of $m$ real-valued objective functions which are either continuous or discrete.
$G(X)$ and $H(X)$ are the constraint vectors, which consists of real-valued functions representing inequality and equality constraints, respectively.

==> Equations/DMOO/Opp_Dir.tex <==
\begin{equation}
\label{equ:DMOO/Opp_Dir}
opp_{(k \Rightarrow i)} = c_{2i-k}
\end{equation}
In Equation \ref{equ:DMOO/Opp_Dir},\\
$opp_{(k \Rightarrow i)}$ is the opposite direction of cell $c_k$ with reference to the centre point $c_i$.

==> Equations/DMOO/Physarum_AA.tex <==
\begin{equation}
\label{equ:DMOO/phy_aa}
    P\_AA_{P_{i} \to P_{k}}  =
    \begin{cases}
      1, & \text{if}\ P_{k}~\text{is Empty} \\
      1, & \text{if}\ ~PID_{i} = PID_{k} \\
      0, & \text{otherwise}
    \end{cases}
\end{equation}
In Equation \ref{equ:DMOO/phy_aa},\\
%$P\_AA_{(i,j),(k,l)}$ defines whether Physarum at cell $c_{(i,j)}$ is available to diffuse towards a neighbouring cell $c_{(k,l)}$.\\
$PID_{i}$ is the ID of the Physarum $P_{i}$.

==> Equations/DMOO/Physarum_AttForce.tex <==
\begin{equation}
\label{equ:DMOO/phy_attforce}
\begin{multlined}
P\_AttForce_{P_{i} \to P_{k}}
= \sum^{F}_{f_i} \left \{
    \dfrac{f_i.Max - f_i(P_{k})}{f_i.Max - f_i.Min}
  \right \}
\end{multlined}
\end{equation}
In Equation \ref{equ:DMOO/phy_attforce},\\
%$P\_AttForce_{(i,j),(k,l)}$ defines the value of attraction force applied on $p.mass_{(i,j)}$ coming from its neighbouring cell $c_{(k,l)}$.\\
$f_i.Min$ and $f_i.Max$ is the local minimum / maximum value (local to Physarum) for objective function $f_i$ respectively.

==> Equations/DMOO/Physarum_Diff.tex <==
\begin{equation}
\label{equ:DMOO/phy_diff}
  \begin{multlined}
   PM^{t+1}_{i} = PM^{t}_{i} +\\
   \sum_{P_{k}}^{NB_{P_{i}}} \left \{
    \begin{aligned}
      & \big(PF * PD\big) \big(PM^{t}_{k} - PM^{t}_{i}\big) && \text{if}\ P\_AA_{P_{i} \to P_{k}} = 1, \\ 
       & && \hspace{0.25cm} PM^{t}_{i} > Diff\_Thr\\
       &0, && \text{otherwise}
     \end{aligned} \right \}.
 \end{multlined}
\end{equation}
The variables in Equation \ref{equ:DMOO/phy_diff} are explained as follows:\\
$PM^{t+1}_{i}$ defines the diffusion of Physarum $P_{i}$ mass for the next iteration $(t+1)$,\\
$PM^{t}_{i}$ is the current mass of Physarum $P_{i}$ for iteration $(t)$,\\
$PM^{t}_{k}$ is the current mass of neighbouring Physarum $P_{k}$,\\
$NB_{P_{i}}$ is the neighbourhood of Physarum $P_{i}$ as in Definition \ref{equ:DMOO/Physarum_Neighbourhood}
$PF$ is the sum of forces affecting Physarum diffusion (Defined in Equation \ref{equ:DMOO/phy_forces}),\\
$PD$ is the Physarum diffusion coefficient (Defined in Equation \ref{equ:DMOO/phy_df}),\\
$P\_AA_{P_{i} \to P_{k}}$ indicates whether Physarum $P_{i}$ is available to diffuse towards a neighbouring Physarum $P_{k}$ (Defined in Equation \ref{equ:DMOO/phy_aa}),\\
$Diff\_Thr$ is the threshold in which the Physarum mass must exceed in order to diffuse.
\begin{equation}
\label{equ:DMOO/phy_df}
PD = \dfrac{nbSize}{10^n}
\end{equation}
In Equation \ref{equ:DMOO/phy_df},\\
$nbSize$ is the neighbourhood's size of Physarum $P_{i}$ (Definition \ref{equ:DMOO/Physarum_Neighbourhood})\\
$n$ is the dimensionality of the problem space.
\begin{equation}
\label{equ:DMOO/phy_forces}
PF = 1 + P\_AttForce_{P_{i} \to P_{k}} + P\_RepForce_{P_{i} \gets P_{k}}
\end{equation}
In Equation \ref{equ:DMOO/phy_forces},\\
$P\_AttForce_{P_{i} \to P_{k}}$ defines the value of attraction forces applied on Physarum $P_{i}$ coming from its neighbouring Physarum $P_{k}$ (Defined in Equation \ref{equ:DMOO/phy_attforce}).\\
$P\_RepForce_{P_{i} \gets P_{k}}$ defines the value of repulsion forces applied on Physarum $P_{i}$ exerted by its neighbouring Physarum $P_{k}$ (Defined in Equation \ref{equ:DMOO/phy_repforce}).

==> Equations/DMOO/Physarum_RepForce.tex <==
\begin{equation}
\label{equ:DMOO/phy_repforce}
\begin{multlined}
P\_RepForce_{P_{i} \gets P_{k}}\\
= \left \{
  \begin{aligned}
    & \dfrac{PM_{opp_{(k \Rightarrow i)}}}{Total\_Physarum\_Mass} && \text{if}\ PID_{i} \neq PID_{opp_{(k \Rightarrow i)}},\\ 
    & && \hspace{0.25cm} PM_{opp_{(k \Rightarrow i)}} > Rep\_Thr\\
    &0, && \text{otherwise}
  \end{aligned} \right.
\end{multlined}
\end{equation}
In Equation \ref{equ:DMOO/phy_repforce},\\
%$P\_RepForce_{(i,j),(k,l)}$ defines the value of repulsion force applied on $p.mass_{(i,j)}$ exerted by its neighbouring Physarum $p.mass_{(k,l)}$.\\
$PM_{opp_{(k \Rightarrow i)}}$ is the neighbour Physarum mass at the opposite direction of Physarum $P_{k}$ with reference to the centre point $c_{i}$ as defined in Equation \ref{equ:DMOO/Opp_Dir}.\\
$Rep\_Thr$ is a threshold where Physarum must reach to repel neighbouring Physarum.

==> Equations/Model/CHM_AA.tex <==
\begin{equation}
\label{equ:Model/chm_aa}
    C\_AA_{(i,j),(k,l)} =
    \begin{cases}
      0, & \text{if}\ CT_{(k,l)} = "OBSTACLE" \\
      1, & \text{otherwise}
    \end{cases}
\end{equation}
where $CT_{(k,l)}$ represents the cell type as defined in Equation \ref{equ:Model/Cell_Type}).

==> Equations/Model/CHM_Diff.tex <==
\begin{equation}
\label{equ:Model/chm_diff}
\begin{multlined}
CM^{t+1}_{(i,j)} = CM^{t}_{(i,j)} +\\
\sum_{(k,l)} \left \{
  \begin{aligned}
    & CD * (CM^{t}_{(k,l)} - CM^{t}_{(i,j)}) && \text{if}\ C\_AA_{(i,j),(k,l)} = 1\\ 
    &0 && \text{otherwise}
  \end{aligned} \right.
\end{multlined}
\end{equation}
\begin{equation*}
\begin{multlined}
  \begin{aligned}
  &\forall (k,l) : &&i - 1 \leqslant k \leqslant i + 1,\\
  &				   &&j - 1 \leqslant l \leqslant j + 1,\\
  &                &&k \neq l
  \end{aligned}
\end{multlined}
\end{equation*}

where
$CM^{t+1}_{(i,j)}$ defines the diffusion of chemical mass for the next generation $(t+1)$ at cell $c_{(i,j)}$.\\
$CM^{t}_{(i,j)}$ is the current mass of the chemical at iteration $(t)$ for cell $c_{(i,j)}$.\\
$CM^{t}_{(k,l)}$ is the current mass of the chemical at iteration $(t)$ for neighbouring chemical cell $c_{(k,l)}$.\\
$CD$ is the chemical diffusion coefficient.\\
$C\_AA_{(i,j),(k,l)}$ defines whether chemical at cell $c_{(i,j)}$ is available to diffuse towards a neighbouring cell $c_{(k,l)}$ as defined in Equation \ref{equ:Model/chm_aa}.

==> Equations/Model/Cell_Type.tex <==
\begin{equation}
\label{equ:Model/Cell_Type}
%CT_{(i, j)} = \left\{
%\begin{matrix}
%FREE \\ OBSTACLE \\ PHYSARUM \\ CHEMICAL
%\end{matrix}
%\right\}
CT_{(i, j)} = \{"FREE", "OBSTACLE", "PHYSARUM", "CHEMICAL"\}
\end{equation}
%CT_{(i, j)} = \{"FREE", "OBSTACLE", "PHYSARUM", "CHEMICAL"\}
where $CT_{(i,j)}$ represents the cell type.

==> Equations/Model/Diffusion_Equation.tex <==
%\begin{equation}
\begin{gather*}
\label{equ:Model/Diffusion_Equation}
   u^{t+1}_{(i,j)} = u^{t}_{(i,j)} + \sum_{k,l} \left \{D (u^{t}_{(k,l)} - u^{t}_{(i,j)}) \right \}.\\
   \forall (k,l):~i - 1 \leqslant k \leqslant i + 1,\\ 
   j - 1 \leqslant l \leqslant j + 1,\\
   k \neq l
\end{gather*}
%\end{equation}

In the above, $u^{t+1}_{(i,j)}$ is the density of the diffusing material (in our case Physarum and/or Chemical) at time $t+1$ located at $(i,j)$, $D$ is the diffusion coefficient and determines how fast $u$ changes in time, $u^{t}_{(k,l)}$ is the material (in our case Physarum and/or Chemical) at one of the adjacent hexagonal neighbours.

==> Equations/Model/Diffusion_Equation_Original.tex <==
\begin{equation}
\label{equ:Model/Diffusion_Equation_Original}
  \frac{\partial u(\mathbf{x},t)}{\partial t} = D\nabla^2u(\mathbf{x},t), 
\end{equation}
where $u(\mathbf{x},t)$ is the density of the diffusing material, $\mathbf{x}$ is a coordinate in space, and $t$ is time. The coefficient $D$ is the diffusion coefficient and determines how fast $u$ changes in time. This equation is also called the \textit{heat equation}, which describes the distribution of heat in a given region over time.

==> Equations/Model/Opp_Dir.tex <==
\begin{equation}
\label{equ:Model/Opp_Dir}
Opp\_Dir_{(i,j) \Leftarrow (k,l)} = c_{(2i-k~,~2j-l)}
\end{equation}
%CT_{(i, j)} = \{"FREE", "OBSTACLE", "PHYSARUM", "CHEMICAL"\}
where $Opp\_Dir_{(i,j) \Leftarrow (k,l)}$ is the opposite direction of cell $c_{(k,l)}$ with reference to the centre point $c_{(i,j)}$.

==> Equations/Model/SM_AA.tex <==
\begin{equation}
\label{equ:Model/sm_aa}
    P\_AA_{(i,j),(k,l)} =
    \begin{cases}
      1, & \text{if}\ CT_{(k,l)} = "FREE" \\
      1, & \text{if}\ CT_{(k,l)} = "PHYSARUM",\\
         & ~PID_{(i,j)} = PID_{(k,l)} \\
      0, & \text{otherwise}
    \end{cases}
\end{equation}

where
$CT_{(k,l)}$ represents the cell type as defined in Equation \ref{equ:Model/Cell_Type}.\\
$PID_{(i,j)}$ is the ID of the Physarum at cell $c_{(i,j)}$.\\

==> Equations/Model/SM_AttForce.tex <==
\begin{equation}
\label{equ:Model/sm_attforce}
\begin{multlined}
P\_AttForce^{t}_{(i,j),(k,l)} = \\
\left \{
  \begin{aligned}
    &WM_{(i,j)} * \dfrac{CM^{t}_{(k,l)}}{Total\_NCM_{(i,j)}} + WQ_{(i,j)} * \dfrac{CQ^{t}_{(k,l)}}{Total\_NCQ_{(i,j)}}, \\
    & \hspace{3cm} \text{if}\ CM^{t}_{(k,l)} = MAX(CM^{t}_{(i,j)})\\
    &0, \hspace{5cm} \text{otherwise}
  \end{aligned} \right.
\end{multlined}
\end{equation}
\begin{equation*}
\begin{multlined}
WM_{(i,j)} = \dfrac{PH^{t}_{(i,j)}}{100},
WQ_{(i,j)} = \dfrac{100 - PH^{t}_{(i,j)}}{100}
\end{multlined}
\end{equation*}

where
$P\_AttForce_{(i,j),(k,l)}$ defines the value of attraction forces applied on Physarum at cell $c_{(i,j)}$ coming from its neighbouring cell $c_{(k,l)}$.\\
$WM_{(i,j)}$ is the weight assigned to the chemical mass that will attract Physarum to it.\\
$CM^{t}_{(k,l)}$ is the current mass of the chemical at iteration $(t)$ for cell $c_{(k,l)}$.\\
$Total\_NCM_{(i,j)}$ is the total summation of chemical mass for the first neighbour of cell $c_{(i,j)}$.\\
$WQ_{(i,j)}$ is the weight assigned to the chemical quality that will attract Physarum to it.\\
$CQ^{t}_{(k,l)}$ is the current quality of chemical at iteration $(t)$ for cell $c_{(k,l)}$, where $CQ \in [0-10]$; 0: Low quality, 10: High quality.\\
$Total\_NCQ_{(i,j)}$ is the total summation of chemical quality for the first neighbour of cell $c_{(i,j)}$.\\
$MAX(CM^{t}_{(i,j)})$ is a function which returns the maximum value of chemical mass among the neighbourhood of cell $c_{(i,j)}$.\\
$PH_{(i,j)}$ is the hunger motivation of the Physarum, where $PH \in [0-100]$; 0:Satiated, 100:Hungry.\\

==> Equations/Model/SM_Diff.tex <==
\begin{equation}
\label{equ:Model/sm_diff}
\begin{multlined}
   PM^{t+1}_{(i,j)} = PM^{t}_{(i,j)} +\\
   \sum_{(k,l)} \left \{
    \begin{aligned}
      & (PF * PD) (PM^{t}_{(k,l)} - PM^{t}_{(i,j)}) \\ 
       & \hspace{3cm}  \text{if}\ P\_AA_{(i,j),(k,l)} = 1, \\
       & \hspace{3cm} PM^{t}_{(i,j)} > Diff\_limit\\
       &0, \hspace{2.7cm} \text{otherwise}
     \end{aligned} \right.
\end{multlined}
\end{equation}
\begin{equation*}
   \begin{aligned}
   &\forall (k,l) : &&i - 1 \leqslant k \leqslant i + 1,\\
   &				   &&j - 1 \leqslant l \leqslant j + 1,\\
    &                &&k \neq l
   \end{aligned}
\end{equation*}
\begin{equation*}
PF = 1 + P\_AttForce_{(i,j),(k,l)} + P\_RepForce_{(i,j),(k,l)}
\end{equation*}

where
$PM^{t+1}_{(i,j)}$ defines the diffusion of Physarum mass for the next generation $(t+1)$ at cell $c_{(i,j)}.$\\
$PM^{t}_{(i,j)}$ is the current mass of Physarum at cell $c_{(i,j)}$.\\
$PM^{t}_{(k,l)}$ is the current mass of neighbouring Physarum at cell $c_{(k,l)}$.\\
$P\_AA^{t}_{(i,j),(k,l)}$ defines whether Physarum at cell $c_{(i,j)}$ is available to diffuse towards a neighbouring cell $c_{(k,l)}$ as defined in Equation \ref{equ:Model/sm_aa}.\\
$PD$ is the Physarum diffusion coefficient.\\
$Diff\_Limit$ is the limit which in which the Physarum mass must exceed in order to diffuse.\\
$PF$ is the sum of forces affecting Physarum.\\
%$P\_AttForce_{(i,j),(k,l)}$ defines the value of attraction forces applied on Physarum at cell $c_{(i,j)}$ coming from its neighbouring cell $c_{(k,l)}$ as defined in Equation \ref{equ:Model/sm_attforce}.\\
%$P\_RepForce_{(i,j),(k,l)}$ defines the value of repulsion forces applied on Physarum at cell $c_{(i,j)}$ exerted by its neighbouring cell $c_{(k,l)}$ as defined in Equation \ref{equ:Model/sm_repforce}.\\

==> Equations/Model/SM_DiffOther.tex <==
\begin{equation}
 \label{equ:Model/smdiff}
 \begin{multlined}
  SM^{t+1}_{(i,j)} = SM^{t}_{(i,j)} +\\
  \sum_{(k,l)} \left \{
   \begin{aligned}{}
      &\big(SF * SD * SM^{t}_{(k,l)}\big) - SM^{t}_{(i,j)} \hspace{0.15cm} \\ &\text{if}\ SM\_AA_{(k,l)} = 1,\\ 
&SM^{t}_{(i,j)} > Diff\_limit \hspace{0.10cm}0, \\ 
 &\text{otherwise}
    \end{aligned} \right.
  \\
   \begin{aligned}{}
    &\forall (k,l) : &&i - 1 \leqslant k \leqslant i + 1,\\
   &				   &&j - 1 \leqslant l \leqslant j + 1,\\
    &                &&k \neq l
    \end{aligned}
  \\
  \\
  SF = 1 + SM\_AttForce^{t}_{(i,j),(k,l)} + SM\_RepForce^{t}_{(i,j),(k,l)}
 \end{multlined}
 \end{equation}

==> Equations/Model/SM_RepForce.tex <==
\begin{equation}
\label{equ:Model/sm_repforce}
\begin{multlined}
P\_RepForce^{t}_{(i,j),(k,l)} = \\
\left \{
  \begin{aligned}
    & \dfrac{PM^{t}_{(2i-k~,~2j-l)}}{Total\_NPM_{(i,j)}} && \text{if}\ PID_{(i,j)} \neq PID_{(2i-k~,~2j-l)},\\
    & && \hspace{0.25cm} PM^{t}_{(2i-k~,~2j-l)} > Rep\_Limit\\
    &0, && \text{otherwise}
  \end{aligned} \right.
\end{multlined}
\end{equation}

where
$P\_RepForce_{(i,j),(k,l)}$ defines the value of repulsion forces applied on Physarum at cell $c_{(i,j)}$ exerted by its neighbouring cell $c_{(k,l)}$.\\
$PM^{t}_{(2i-k~,~2j-l)}$ is the neighbour Physarum mass at the opposite direction of cell $c_{(k,l)}$ with reference to the centre point $c_{(i,j)}$ as defined in Equation \ref{equ:Model/Opp_Dir}.\\
$Total\_NPM_{(i,j)}$ is is the total summation of Physarum mass for the first neighbour of cell $c_{(i,j)}$.\\
$Rep\_Limit$ is a limit where Physarum must reach to repel neighbouring Physarum.\\

==> Equations/WSN/S_AA.tex <==
\begin{equation}
\label{equ:WSN/s_aa}
    S\_AA_{(i,j),(k,l)} =
    \begin{cases}
      1, & \text{if}\ CT_{(k,l)} = "FREE"~OR~"INTEREST\_POINT"\\
      1, & \text{if}\ CT_{(k,l)} = ("SENSOR")~AND~(SID_{(i,j)} = SID_{(k,l)})\\
      0, & \text{otherwise}
    \end{cases}
\end{equation}
where
$S\_AA_{(i,j),(k,l)}$ defines whether an actor at cell $c_{(i,j)}$ is available to diffuse towards a neighbouring cell $c_{(k,l)}$.\\
$SID_{(i,j)}$ is the ID of the sensor.\\

==> Equations/WSN/S_AttForce.tex <==
\begin{equation}
\label{equ:WSN/s_attforce}
\begin{multlined}
S\_AttForce_{(i,j),(k,l)} =
  \begin{cases}
    \dfrac{IPM_{(k,l)}}{Total\_IPM}, & \text{if}\ IPM_{(k,l)} = MAX(IPM_{(i,j)})\\ 
    0, & \text{otherwise}
  \end{cases}
\end{multlined}
\end{equation}
where
$S\_AttForce_{(i,j),(k,l)}$ defines the value of attraction force of $SE_{(i,j)}$ towards its neighbouring cell $c_{(k,l)}$.\\
$IPM_{(i,j)}$ is the current mass of the interest point for cell $c_{(i,j)}$.\\
$Total\_IPM$ is the total sum of all interest points mass on the grid.\\

==> Equations/WSN/S_Diff.tex <==
\begin{equation}
 \label{equ:WSN/s_diff}
 \begin{multlined}
  SE^{t+1}_{(i,j)} = SE^{t}_{(i,j)} + \sum_{(k,l)}
   \begin{cases}
      \big(SF * SD * SE^{t}_{(k,l)}\big) - SE^{t}_{(i,j)}, &\text{if}\ S\_AA_{(i,j),(k,l)} = 1\\
      0, & \text{otherwise}
    \end{cases}
\\
\noindent \hfill
\begin{aligned} 
\forall (k,l):~&i - 1 \leqslant k \leqslant i + 1,\\ 
&j - 1 \leqslant l \leqslant j + 1,\\
&k \neq l\\
\end{aligned}
\\
\noindent
SF = 1 + S\_AttForce^{t}_{(i,j),(k,l)} + S\_RepForce^{t}_{(i,j),(k,l)}
\hfill
\end{multlined}
\end{equation}
where
$SE^{t+1}_{(i,j)}$ defines the diffusion of actor energy for the next generation $(t+1)$ at cell $c_{(i,j)}$.\\
$SE^{t}_{(i,j)}$ is the current energy of an actor at iteration $(t)$ for cell $c_{(i,j)}$.\\
$SF$ is the forces affecting an actor.\\
$SD$ is the actor diffusion coefficient.\\



==> Equations/WSN/S_RepForce.tex <==
\begin{equation}
\label{equ:WSN/s_repforce}
\begin{multlined}
S\_RepForce_{(i,j),(k,l)} =
  \begin{cases}
    \dfrac{SE^{t}_{opp(k,l)}}{Total\_SE}, & \text{if}\ SID_{(i,j)} \neq SID_{opp(k,l)},\\ 
    & \hspace{0.27cm} SE^{t}_{opp(k,l)} > Rep\_Limit\\
    0, & \text{otherwise}
  \end{cases}
\end{multlined}
\end{equation}
where
$S\_RepForce_{(i,j),(k,l)}$ defines the value of repulsion force of $SE_{(i,j)}$ towards its neighbouring cell $c_{(k,l)}$.\\
$SE^{t}_{opp(i,j)}$ is the neighbour sensor energy at the opposite direction.\\
$Rep\_Limit$ is a limit where a sensor must reach to repel a neighbouring sensor.\\

==> Equations/WSN/WSN_Problem_Def.tex <==
\begin{equation}
\label{equ:WSN/WSN_Problem_Def}
\begin{aligned}
& G = (V,E)\\
& V = \{v_1, v_2, \ldots , v_n\} \\
& E \subseteq \{e_{(x,y)} \: | \: (x,y) \in V^2 \: \land \: x \neq y\}  \\
\end{aligned}
\end{equation}
In the above equation,
$V$ is the set of sensor nodes, and $E$ is a set of edges established between every two nodes.

==> Figures/DMOO/DV_Box_Plot.tex <==
\begin{figure*}
\begin{center}
\includegraphics[scale=0.9]{Figures/DMOO/DV_Box_Plot.png}
\caption{Box-Plot graph of performance indicators for our PCA algorithms and the four state-of-the-art MOEAs with respect to Deep Valley problem.}
\label{fig:DMOO/DV_Box_Plot}
\end{center}
\end{figure*}

==> Figures/DMOO/PCA_DMOO.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/DMOO/PCA_DMOO.png}
\caption{(a) Physarum search space is mapped to the (b) objective space, in which each cell in the search space is decoded as a food resource to attract Physarum (This figure is based on \cite{RefWorks:352} with modifications).}
\label{fig:DMOO/PCA_DMOO}
\end{figure*}

==> Figures/DMOO/Quality_Indicators.tex <==
\begin{figure*}
\begin{center}
\includegraphics[scale=0.7]{Figures/DMOO/Quality_Indicators.png}
\caption{Quality indicators classification based on which aspect they measure \cite{RefWorks:284}.}
\label{fig:DMOO/Quality_Indicators}
\end{center}
\end{figure*}

==> Figures/DMOO/TPF.tex <==
\begin{figure*}
\begin{center}
\includegraphics[scale=0.7]{Figures/DMOO/TPF.png}
\caption{In this DMOO problem, we are trying to maximise the performance and at the same time minimise the cost. The red dots are the non-dominated solution (Pareto front) while the yellow dots are example of solutions dominated by red ones (This figure is based on \cite{RefWorks:352} with some modifications).}
\label{fig:DMOO/TPF}
\end{center}
\end{figure*}

==> Figures/DMOO/nD_Hex.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/DMOO/nD_Hex.png}
\caption{A bcc voxel, its 8-neighbourhood and 14-neighbourhood \cite{RefWorks:297}.}
\label{fig:DMOO/nD_Hex}
\end{figure*}

==> Figures/Introduction/Bioinspired_Algorithm_Steps.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Introduction/Bioinspired_Algorithm_Steps.png}
\caption{Three steps to develop Physarum-inspired algorithm.}
\label{fig:Introduction/Bioinspired_Algorithm_Steps}
\end{figure*}

==> Figures/Introduction/Framework.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth]{Figures/Introduction/Framework.png}
\caption{Research Framework.}
\label{fig:Introduction/Framework}
\end{figure*}

==> Figures/Literature_Review/Physarum_Agent_Model.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Literature_Review/Physarum_Agent_Model.png}
\caption{The architecture and morphology of an agent \cite{RefWorks:84}.}
\label{fig:Literature_Review/Physarum_Agent_Model}
\end{figure*}

==> Figures/Literature_Review/Physarum_Chip.tex <==
\begin{figure*}[t!]
\includegraphics[width=\textwidth, height=\textheight/2]{Figures/Literature_Review/Physarum_Chip.png}
\caption{Physarum Chip \cite{RefWorks:326}.}
\label{fig:Literature_Review/Physarum_Chip}
\end{figure*}

==> Figures/Literature_Review/Physarum_Competition.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Literature_Review/Physarum_Competition.png}
\caption{Experiment with two agents: Physarum polycephalum could grow into branches of Badhamiautricularis \cite{RefWorks:316}.}
\label{fig:Literature_Review/Physarum_Competition}
\end{figure*}

==> Figures/Literature_Review/Physarum_Maze_Solving.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Literature_Review/Physarum_Maze_Solving.png}
\caption{Maze-solving by Physarum polycephalum \cite{RefWorks:66}.}
\label{fig:Literature_Review/Physarum_Maze_Solving}
\end{figure*}

==> Figures/Literature_Review/Physarum_Tokyo_railway_network.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[scale=0.6]{Figures/Literature_Review/Physarum_Tokyo_railway_network.png}
\caption{Tokyo rail network formation with Physarum polycephalum \cite{RefWorks:67}.}
\label{fig:Literature_Review/Physarum_Tokyo_railway_network}
\end{center}
\end{figure*}

==> Figures/Literature_Review/Physarum_living_CA.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[scale=0.95]{Figures/Literature_Review/Physarum_living_CA.png}
\caption{Physarum living cellular automatons \cite{RefWorks:68}}
\label{fig:Literature_Review/Physarum_living_CA}
\end{center}
\end{figure*}

==> Figures/Literature_Review/Physarum_memristor.tex <==
\begin{figure*}
\includegraphics[width=\textwidth, height=\textheight/2]{Figures/Literature_Review/Physarum_memristor.png}
\caption{(a) Petri dish set up for chemotactic assessment before growth. (b) Petri dish with correct growth of Physarum polycephalum, connected for electrical potential recording. (c) Example of protoplasmic tube growth\cite{RefWorks:122}.}
\label{fig:Literature_Review/Physarum_memristor}
\end{figure*}

==> Figures/Model/Cell_Diffusion_Process.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Cell_Diffusion_Process.png}
\caption{Cell Diffusion Process.}
\label{fig:Model/Cell_Diffusion_Process}
\end{figure*}

==> Figures/Model/Diffusion_on_CA.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Diffusion_on_CA.png}
\caption{The structure of the cellular automaton and how diffusion process is executed over time.}
\label{fig:Model/Diffusion_on_CA}
\end{figure*}

==> Figures/Model/Filled_Grid.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Filled_Grid.png}
\caption{An example of a grid of four Physarum competing for two food resources, some obstacles and empty cells.}
\label{fig:Model/Filled_Grid}
\end{figure*}

==> Figures/Model/Heuristic_R1.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Heuristic_R1.png}
\caption{\textit{Heuristic Rule 1}: A cell occupied by a Chemical (e.g. food source(s)) and/or a Physarum diffuses in all available neighbourhood.}
\label{fig:Model/Heuristic_R1}
\end{figure*}

==> Figures/Model/Heuristic_R2.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Heuristic_R2.png}
\caption{\textit{Heuristic Rule 2}: A cell can be occupied by one or more chemical class and by at most one Physarum in each cell \cite{RefWorks:346}.}
\label{fig:Model/Heuristic_R2}
\end{figure*}

==> Figures/Model/Heuristic_R3.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Heuristic_R3.png}
\caption{\textit{Heuristic Rule 3}: Chemo attraction forces exerted on Physarum will be a function of chemical having different mass and quality \cite{RefWorks:56,RefWorks:67,RefWorks:58} and Physarum hunger motivation \cite{RefWorks:308}. If Physarum is satisfied, it would appreciate the quality of chemical rather than the mass, and the opposite if it is hungry.}
\label{fig:Model/Heuristic_R3}
\end{figure*}

==> Figures/Model/Heuristic_R4.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Heuristic_R4.png}
\caption{\textit{Heuristic Rule 4}: Competing Physarum will exert repulsion forces on each other which will be calculated as a negative force \cite{RefWorks:346}.}
\label{fig:Model/Heuristic_R4}
\end{figure*}

==> Figures/Model/Heuristic_R5.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Heuristic_R5.png}
\caption{\textit{Heuristic Rule 5}: When two Physarum are competing for the same cell, the one with the higher power (mass) will occupy it \cite{RefWorks:316}.}
\label{fig:Model/Heuristic_R5}
\end{figure*}

==> Figures/Model/Heuristic_R6.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Heuristic_R6.png}
\caption{\textit{Heuristic Rule 6}: A food resource engulfed by a Physarum will be excluded, and this Physarum mass will grow at this point according to this food resource quality}
\label{fig:Model/Heuristic_R6}
\end{figure*}

==> Figures/Model/Heuristic_R7.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Heuristic_R7.png}
\caption{\textit{Heuristic Rule 7}: In the Physarum exploration phase, if the mass of the Physarum is less than a critical value the Physarum will stop diffusing to prevent the Physarum from spreading all over the board (as exhibited by Physarum in biological experiments).}
\label{fig:Model/Heuristic_R7}
\end{figure*}

==> Figures/Model/Heuristic_R8.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Heuristic_R8.png}
\caption{\textit{Heuristic Rule 8}: In the Physarum exploitation phase, based on the feedback phenomenon \cite{RefWorks:66}, the protoplasmic flux to the high-quality food source tends to increment, while the protoplasmic flux to poor quality food source tends to decrement, and will potentially vanish. Thus Physarum tend to shrink and collect its body mass to move towards resource of attraction.}
\label{fig:Model/Heuristic_R8}
\end{figure*}

==> Figures/Model/Hex.tex <==
\begin{figure*}[t!]
\includegraphics[width=\textwidth]{Figures/Model/Hex.png}
\caption{Hexagonal neighbourhood.}
\label{fig:Model/Hex}
\end{figure*}

==> Figures/Model/Hex_Coordinates.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth/2]{Figures/Model/Hex_Coordinates.png}
\caption{even-row horizontal layout shoves even rows right \cite{RefWorks:335}.}
\label{fig:Model/Hex_Coordinates}
\end{center}
\end{figure*}

==> Figures/Model/Model_EXP1A_BOX_PLOT.tex <==
\begin{figure*}[t!]
\begin{center}
\includegraphics[scale=0.7]{Figures/Model/Model_EXP1A_BOX_PLOT.png}
\caption{Represents the first setting (A) of Experiment (I) where Physarum of higher mass (P1) engulfed more food resources than Physarum of lower mass (P2).}
\label{fig:Model/Model_EXP1A_BOX_PLOT}
\end{center}
\end{figure*}

==> Figures/Model/Model_EXP1B_BOX_PLOT.tex <==
\begin{figure*}[t!]
\begin{center}
\includegraphics[scale=0.7]{Figures/Model/Model_EXP1B_BOX_PLOT.png}
\caption{Represents the second setting (B) of Experiment (I) where Physarum started and ended engulfing food resources of high quality (F1) faster than food resources of low quality (F2) as indicated by less number of iterations.}
\label{fig:Model/Model_EXP1B_BOX_PLOT}
\end{center}
\end{figure*}

==> Figures/Model/Model_Exp1A.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Model_Exp1A.png}
\caption{An example grid of Experiment (I) setting (A).}
\label{fig:Model/Model_Exp1A}
\end{figure*}

==> Figures/Model/Model_Exp1AB.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Model_Exp1AB.png}
\caption{An example grid of Experiment (I) setting (A) and (B).}
\label{fig:Model/Model_Exp1AB}
\end{figure*}

==> Figures/Model/Model_Exp1B.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/Model/Model_Exp1B.png}
\caption{An example grid of Experiment (I) setting (B).}
\label{fig:Model/Model_Exp1B}
\end{figure*}

==> Figures/Model/Model_Exp2_Territory.tex <==
\begin{figure*}
\begin{center}
\includegraphics[scale=0.5]{Figures/Model/Model_Exp2_Territory.png}
\caption{Graphical simulation of 10 Physarum foraging behaviour in competition settings after engulfing all food resources, where yellow cells indicate engulfed food resource and the number inside indicates Physarum (ID) engulfed this food resource, white cells indicate empty cells and other coloured cells indicate Physarum and the number inside indicates the ID of the Physarum (ranging from $1$ to $10$) and their mass range from $1,000$ to $10,000$ respectively.}
\label{fig:Model/Model_Exp2_Territory}
\end{center}
\end{figure*}

==> Figures/Model/Model_State.tex <==
\begin{figure*}
\begin{center}
\includegraphics[scale=0.4]{Figures/Model/Model_State.png}
\caption{Model State.}
\label{fig:Model/Model_State}
\end{center}
\end{figure*}

==> Figures/Model/System_Evolution_Process.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth,height=\textheight,keepaspectratio]{Figures/Model/System_Evolution_Process.png}
\caption{System Evolution Process.}
\label{fig:Model/System_Evolution_Process}
\end{center}
\end{figure*}

==> Figures/Model/Von_Moore.tex <==
\begin{figure*}[t!]
\includegraphics[width=\textwidth]{Figures/Model/Von_Moore.png}
\caption{Von Neumann / Moore neighbourhoods.}
\label{fig:Model/Von_Moore}
\end{figure*}

==> Figures/WSN/Exp1_Results.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/WSN/Exp1_Results.png}
\caption{(a) Movement steps and (b) Area coverage versus number of rounds for the three scenarios.}
\label{fig:WSN/Exp1_Results}
\end{figure*}

==> Figures/WSN/Exp1_Simulation.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/WSN/Exp1_Simulation.png}
\caption{(a) The initial sensor deployment and (b) the relocation of sensors after 30 round execution of the proposed algorithm for the first scenario (82 sensors).}
\label{fig:WSN/Exp1_Simulation}
\end{figure*}

==> Figures/WSN/Exp2A_Simulation.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/WSN/Exp2A_Simulation.png}
\caption{(a) The initial network simulation with a total nodes of 100 and $R_c=5$, and (b) after algorithm execution (with k-influence) to get a connected network.}
\label{fig:WSN/Exp2A_Simulation}
\end{figure*}

==> Figures/WSN/Exp2B_Simulation.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/WSN/Exp2B_Simulation.png}
\caption{(a) The network simulation after random elimination of 50 nodes (total remaining nodes is 50), and (b) after algorithm execution (with k-influence) to get a connected network.}
\label{fig:WSN/Exp2B_Simulation}
\end{figure*}

==> Figures/WSN/Exp2_Results.tex <==
\begin{figure*}
\begin{center}
\includegraphics[scale=0.65]{Figures/WSN/Exp2_Results.png}
\caption{In experiment II, two algorithms were applied. First was using the concept of regions of the k-influence (blue line) and the second without this concept (red line), where (a) is the total moving distance, (b) is the number of relocated nodes, and (c) is the average movement per node after randomly eliminating [10\%, 20\%, \dots, 90\%] of actor nodes and applying the fault repair algorithm after each elimination.}
\label{fig:WSN/Exp2_Results}
\end{center}
\end{figure*}

==> Figures/WSN/Hex_Tessellation.tex <==
\begin{figure*}
\centering
\includegraphics[]{Figures/WSN/Hex_Tessellation.png}
\caption{The area will be dynamically tessellated by regular hexagons with its side equal to communication radius ($R_c$) of the sensor. The centres of the regular hexagons will be identified as the interest points to attract mobile sensors.}
\label{fig:WSN/Hex_Tessellation}
\end{figure*}

==> Figures/WSN/MWSN.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/WSN/MWSN.png}
\caption{Mobile Wireless Sensor Networks (MWSN).}
\label{fig:WSN/MWSN}
\end{figure*}

==> Figures/WSN/Node_Failure_Example.tex <==
%\begin{figure*}
%\includegraphics[width=\textwidth]{Figures/WSN/Problem_illustration.png}
%\caption{Node failure problem illustration.}
%\label{fig:WSN/Problem_illustration}
%\end{figure*}

\begin{figure*}[h!]
\includegraphics[width=\textwidth]{Figures/WSN/Uncritical_Node_Example.png}
\caption{Failures of the yellow actors will not disturb connectivity of other actors, so they are called "Uncritical Node".}
\label{fig:WSN/Uncritical_Node_Example}
\end{figure*}

\begin{figure*}[h!]
\includegraphics[width=\textwidth]{Figures/WSN/Critical_Node_Example.png}
\caption{Failures of the red actors will result in disconnection of other actors, so they are called "Critical Node".}
\label{fig:WSN/Critical_Node_Example}
\end{figure*}

\begin{figure*}[h!]
\includegraphics[width=\textwidth]{Figures/WSN/Cut_Vertex_Node_Example.png}
\caption{Failures of the blue actors will cause the network to be partitioned into disjoint network, so they are called "Cut-Vertex Node".}
\label{fig:WSN/Cut_Vertex_Node_Example}
\end{figure*}

==> Figures/WSN/Sim_Hex_Tessellation.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/WSN/Sim_Hex_Tessellation.png}
\caption{In (a) a simulation of area before tessellation and (b) after applying hexagonal tessellation (Stardew Valley Copyright © 2016-2019 ConcernedApe LLC).}
\label{fig:WSN/Sim_Hex_Tessellation}
\end{figure*}

==> Figures/WSN/Similarities.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/WSN/Similarities.png}
\caption{Similarities between WSN Graph optimisation problem (on the left) and Physarum network optimisation (on the right), where in WSN Graph optimisation problem the green nodes represent sensors and blue nodes represent interest points, while in Physarum network optimisation the green nodes represent Physarum and blue nodes represent food resources.}
\label{fig:WSN/Similarities}
\end{figure*}

==> Figures/WSN/Tessellation_Types.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/WSN/Tessellation_Types.png}
\caption{Three unit polygon (triangle, square, and hexagon) tessellations \cite{RefWorks:175}.}
\label{fig:WSN/Tessellation_Types}
\end{figure*}

==> Figures/WSN/WSAN.tex <==
\begin{figure*}
\includegraphics[width=\textwidth]{Figures/WSN/WSAN.png}
\caption{Wireless Sensor-Actor Networks (WSAN) \cite{RefWorks:192}.}
\label{fig:WSN/WSAN}
\end{figure*}

==> Figures/WSN/WSN_Components.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth]{Figures/WSN/WSN_Components.png}
\caption{The components of a sensor node in a WSN \cite{RefWorks:370}.}
\label{fig:WSN/WSN_Components}
\end{figure*}

==> Figures/WSN/WSN_System_Evolution.tex <==
\begin{figure*}
\centering
\includegraphics[height=0.85\textheight,width=\textwidth,keepaspectratio]{Figures/WSN/WSN_System_Evolution.png}
\caption{System Evolution.}
\label{fig:WSN/WSN_System_Evolution}
\end{figure*}

==> Figures/WSN/kinfluence.tex <==
\begin{figure*}[t!]
\begin{center}
\includegraphics[scale=0.35]{Figures/WSN/kinfluence.png}
\caption{Region of k-influence of base station $B$.}
\label{fig:WSN/kinfluence}
\end{center}
\end{figure*}


==> Tables/DMOO/Algorithms_Parameters.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  	\caption{A Summary of the parameters of the algorithms used in the experiments.}
  	\label{tab:DMOO/Algorithms_Parameters}
    \begin{tabular}{|c|p{21.855em}|}
    \toprule
    \multicolumn{1}{|p{6em}|}{\textcolor[rgb]{ .133,  .133,  .133}{\textbf{Algorithms}}} & \textcolor[rgb]{ .133,  .133,  .133}{\textbf{Parameter Settings}} \\
    \midrule
    PCA-MC & \textcolor[rgb]{ .133,  .133,  .133}{$max\text{-}iter=250, N=100, P_{mass}=3000, \newline{}Diff\_Thr=50, Rep\_Thr=50$} \\
    \midrule
    PCA-LHS & \textcolor[rgb]{ .133,  .133,  .133}{$max\text{-}iter=250, N=100, P_{mass}=3000, \newline{}Diff\_Thr=50, Rep\_Thr=50$} \\
    \midrule
    PCA-MC-RE & \textcolor[rgb]{ .133,  .133,  .133}{$max\text{-}iter=250, restart\text{-}iteration = 10, N=100,\newline{} P_{mass}=3000, Diff\_Thr=50, Rep\_Thr=50$} \\
    \midrule
    PCA-LHS-RE & \textcolor[rgb]{ .133,  .133,  .133}{$max\text{-}iter=250, restart\text{-}iteration = 10, N=100,\newline{} P_{mass}=3000, Diff\_Thr=50, Rep\_Thr=50$} \\
    \midrule
    NSGAII & \textcolor[rgb]{ .133,  .133,  .133}{$max\text{-}ev=2500, N=100, P_c=0.9, \eta_c=20.0, \newline{}P_m = 1/d, \eta_m=20.0, OPERATOR=SBXC+PM+BTS$} \\
    \midrule
    NSGAII-45 & \textcolor[rgb]{ .133,  .133,  .133}{$max\text{-}ev=2500, N=100, P_c=0.9, \eta_c=20.0, \newline{}P_m=1/d, \eta_m=20.0, OPERATOR=SBXC+PM+BTS$} \\
    \midrule
    NSGAIII & \textcolor[rgb]{ .133,  .133,  .133}{$max\text{-}iter=250, N=100, P_c=0.9, \eta_c=30.0, \newline{}P_m=1/d, \eta_m=20.0, OPERATOR=SBXC+PM+BTS$} \\
    \midrule
    SPEA2 & \textcolor[rgb]{ .133,  .133,  .133}{$max\text{-}iter=250, N=100, P_c=0.9, \eta_c=20.0, \newline{}P_m=1/d, \eta_m=20.0, OPERATOR=SBXC+PM+BTS$} \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> Tables/DMOO/Algorithms_Rank.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table*}[htbp]
  \centering
  \caption{The mean rank of performance indicators as sorted from the best performance to the worst in an up-down arrangement with respect to all benchmark functions collectively.}
  \label{tab:DMOO/Algorithms_Rank}
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \toprule
    \multicolumn{2}{|c|}{\textbf{HV}} & \multicolumn{2}{c|}{\textbf{IGD+}} & \multicolumn{2}{c|}{\textbf{Epsilon}} & \multicolumn{2}{c|}{\textbf{Spread}} \\
    \midrule
    SPEA2 & 7.24  & PCASwLHS & 2.66  & SPEA2 & 1.86  & PCASwMC & 6.11 \\
    \midrule
    PCASwLHS & 5.63  & PCASwMC & 2.74  & PCASwLHS & 3.41  & PCASwLHS & 5.87 \\
    \midrule
    PCASwMC & 5.51  & SPEA2 & 3.11  & PCASwMC & 3.57  & NSGAII & 4.95 \\
    \midrule
    NSGAII-45 & 4.96  & NSGAII-45 & 4.3   & NSGAII-45 & 4.03  & NSGAII-45 & 4.84 \\
    \midrule
    NSGAII & 4.93  & NSGAII & 4.42  & NSGAII & 4.08  & PCAwMC & 4.33 \\
    \midrule
    NSGAIII & 3.36  & PCAwLHS & 5.97  & NSGAIII & 5.41  & PCAwLHS & 4.3 \\
    \midrule
    PCAwLHS & 2.3   & PCAwMC & 6.13  & PCAwLHS & 6.82  & SPEA2 & 3.03 \\
    \midrule
    PCAwMC & 2.07  & NSGAIII & 6.67  & PCAwMC & 6.84  & NSGAIII & 2.58 \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> Tables/DMOO/All_Problems_Pairwise.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{The statistical pair-wise performance analysis comparing our PCA algorithms versus the 4 state-of-the-art EMO algorithms with respect to all benchmark problems. Three different symbols are used: "$-$" indicates that there is no statistical significance between the algorithms, "$\blacktriangle$" and "$\triangledown$" were used when the algorithm in the column (PCA algorithms) achieves statistically better or worse results, respectively than the algorithm in the row (MOEA algorithms).}
\label{tab:DMOO/All_Problems_Pairwise}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{Problems} & \multicolumn{4}{c|}{NSGAII}                              & \multicolumn{4}{c|}{NSGAII-45}                           & \multicolumn{4}{c|}{NSGAIII}                      & \multicolumn{4}{c|}{SPEA2}                            \\ \cline{2-17} & \rotatebox[origin=c]{90}{HV}        & \rotatebox[origin=c]{90}{IGD+}        & \rotatebox[origin=c]{90}{\epsilon}           & \rotatebox[origin=c]{90}{\Delta}       & \rotatebox[origin=c]{90}{HV}          & \rotatebox[origin=c]{90}{IGD+}        & \rotatebox[origin=c]{90}{\epsilon}           & \rotatebox[origin=c]{90}{\Delta}       & \rotatebox[origin=c]{90}{HV}          & \rotatebox[origin=c]{90}{IGD+}        & \rotatebox[origin=c]{90}{\epsilon}           & \rotatebox[origin=c]{90}{\Delta} 	  & \rotatebox[origin=c]{90}{HV}          & \rotatebox[origin=c]{90}{IGD+}        & \rotatebox[origin=c]{90}{\epsilon}           & \rotatebox[origin=c]{90}{\Delta}           \\ \hline
PCAwMC                    & $\triangledown$ & $\triangledown$ & $\triangledown$ & -              & $\triangledown$ & $\triangledown$ & $\triangledown$ & -              & -              & -              & $\triangledown$ & - & $\triangledown$ & $\triangledown$ & $\triangledown$ & $\triangledown$ \\ \hline
PCAwLHS                   & $\triangledown$ & $\triangledown$ & $\triangledown$ & -              & $\triangledown$ & -           & $\triangledown$ & -              & -              & -              & -           & - & $\triangledown$ & $\triangledown$ & $\triangledown$ & $\triangledown$ \\ \hline
PCASwMC                   & -           & -           & -           & -              & -           & -           & -           & $\blacktriangle$ & -              & $\blacktriangle$ & -           & - & $\triangledown$ & -           & $\triangledown$ & -           \\ \hline
PCASwLHS                  & -           & -           & -           & $\blacktriangle$ & -           & -           & -           & $\blacktriangle$ & $\blacktriangle$ & $\blacktriangle$ & -           & - & -           & -           & -           & -           \\ \hline
\end{tabular}
\end{table*}

%\triangledown
%\blacktriangle


==> Tables/DMOO/Benchmark_Functions.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1 (3)'
\begin{table}[htbp]
  \centering
  \caption{The characteristics of the selected benchmark functions.}
    \begin{tabular}{|c|c|c|c|c|p{8.285em}|p{6.355em}|c|}
    \toprule
    \multicolumn{1}{|p{3.785em}|}{\textbf{Problem\newline{}ID}} & \multicolumn{1}{p{4.715em}|}{\textcolor[rgb]{ .133,  .133,  .133}{\textbf{DMOO\newline{}Problems}}} & \multicolumn{1}{p{1.715em}|}{\textcolor[rgb]{ .133,  .133,  .133}{\textbf{d}}} & \multicolumn{1}{p{1.715em}|}{\textcolor[rgb]{ .133,  .133,  .133}{\textbf{m}}} & \multicolumn{1}{p{1.715em}|}{\textcolor[rgb]{ .133,  .133,  .133}{\textbf{c}}} & \textcolor[rgb]{ .133,  .133,  .133}{\textbf{Discrete variables bounds}} & \textcolor[rgb]{ .133,  .133,  .133}{\textbf{Discrete interval (DI)}} & \textbf{Reference} \\
    \midrule
    1     & ConstrEx & 2     & 2     & 2     & \textcolor[rgb]{ .133,  .133,  .133}{$10<x_0<100$\newline{}$100<x_1<500$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_0) = 0.01$\newline{}$DI(x_1) = 0.01$} & \cite{RefWorks:243} \\
    \midrule
    2     & DTLZ4 & 5     & 3     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<10$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.1$} & \multirow{3}[6]{*}{\cite{RefWorks:272}} \\
\cmidrule{1-7}    3     & DTLZ4 & 2     & 3     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} &  \\
\cmidrule{1-7}    4     & DTLZ4 & 3     & 3     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
    \midrule
    5     & Fonseca & 3     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$-40<x_n<40$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.1$} & \cite{RefWorks:274} \\
    \midrule
    6     & GLT1  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_0<100$\newline{}$-100<x_1<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_0) = 0.01$\newline{}$DI(x_1) = 0.01$} & \multirow{5}[10]{*}{\cite{RefWorks:273}} \\
\cmidrule{1-7}    7     & GLT2  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_0<100$\newline{}$-100<x_1<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_0) = 0.01$\newline{}$DI(x_1) = 0.01$} &  \\
\cmidrule{1-7}    8     & GLT3  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_0<100$\newline{}$-100<x_1<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_0) = 0.01$\newline{}$DI(x_1) = 0.01$} &  \\
\cmidrule{1-7}    9     & GLT4  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_0<100$\newline{}$-100<x_1<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_0) = 0.01$\newline{}$DI(x_1) = 0.01$} &  \\
\cmidrule{1-7}    10    & GLT5  & 3     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_0<50$\newline{}$0<x_1<50$\newline{}$-50<x_2<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_0) = 0.05$\newline{}$DI(x_1) = 0.05$\newline{}$DI(x_2) = 0.05$} &  \\
    \midrule
    11    & Golinski & 7     & 2     & 11    & \textcolor[rgb]{ .133,  .133,  .133}{$26<x_0<36$\newline{}$7<x_1<8$\newline{}$170<x_2<280$\newline{}$73<x_3<83$\newline{}$73<x_4<83$\newline{}$29<x_5<39$\newline{}$50<x_6<55$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_0) = 0.1$\newline{}$DI(x_1) = 0.1$\newline{}$DI(x_2) = 0.1$\newline{}$DI(x_3) = 0.1$\newline{}$DI(x_4) = 0.1$\newline{}$DI(x_5) = 0.1$\newline{}$DI(x_6) = 0.1$} & \cite{RefWorks:301} \\
    \midrule
    12    & MOP1  & 5     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<10$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.1$} & \multirow{4}[8]{*}{\cite{RefWorks:246}} \\
\cmidrule{1-7}    13    & MOP2  & 5     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<10$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.1$} &  \\
\cmidrule{1-7}    14    & MOP3  & 5     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<10$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.1$} &  \\
\cmidrule{1-7}    15    & MOP4  & 5     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<10$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.1$} &  \\
    \bottomrule
    \end{tabular}%
    \label{tab:DMOO/Benchmark_Functions1}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1 (4)'
\begin{table}[htbp]
  \centering
  \caption{The characteristics of the selected benchmark functions.}
    \begin{tabular}{|c|c|c|c|c|p{8.285em}|p{6.285em}|c|}
    \toprule
    \multicolumn{1}{|p{4.215em}|}{\textbf{Problem\newline{}ID}} & \multicolumn{1}{p{4.57em}|}{\textcolor[rgb]{ .133,  .133,  .133}{\textbf{DMOO\newline{}Problems}}} & \multicolumn{1}{p{1.355em}|}{\textcolor[rgb]{ .133,  .133,  .133}{\textbf{d}}} & \multicolumn{1}{p{1.355em}|}{\textcolor[rgb]{ .133,  .133,  .133}{\textbf{m}}} & \multicolumn{1}{p{1.355em}|}{\textcolor[rgb]{ .133,  .133,  .133}{\textbf{c}}} & \textcolor[rgb]{ .133,  .133,  .133}{\textbf{Discrete variables bounds}} & \textcolor[rgb]{ .133,  .133,  .133}{\textbf{Discrete interval (DI)}} & \textbf{Reference} \\
    \midrule
    16    & MOP1  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} & \multirow{12}[24]{*}{\cite{RefWorks:246}} \\
\cmidrule{1-7}    17    & MOP2  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} &  \\
\cmidrule{1-7}    18    & MOP3  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} &  \\
\cmidrule{1-7}    19    & MOP4  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} &  \\
\cmidrule{1-7}    20    & MOP5  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} &  \\
\cmidrule{1-7}    21    & MOP1  & 3     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
\cmidrule{1-7}    22    & MOP2  & 3     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
\cmidrule{1-7}    23    & MOP3  & 3     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
\cmidrule{1-7}    24    & MOP4  & 3     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
\cmidrule{1-7}    25    & MOP5  & 3     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
\cmidrule{1-7}    26    & MOP6  & 3     & 3     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
\cmidrule{1-7}    27    & MOP7  & 3     & 3     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
    \midrule
    28    & NMMin & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$-1000<x_0<1000$\newline{}$-1000<x_1<1000$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_0) = 10$\newline{}$DI(x_1) = 10$} & \cite{RefWorks:302} \\
    \midrule
    29    & Srinivas & 2     & 2     & 2     & \textcolor[rgb]{ .133,  .133,  .133}{$-200<x_n<200$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.1$} & \cite{RefWorks:277} \\
    \midrule
    30    & UF6   & 4     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_0<10$\newline{}$-10<x_n<10$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_0) = 0.1$\newline{}$DI(x_n) = 0.1$} & \cite{RefWorks:300} \\
    \midrule
    31    & Viennet2 & 2     & 3     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$-400<x_n<400$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} & \multirow{2}[4]{*}{\cite{RefWorks:246}} \\
\cmidrule{1-7}    32    & Viennet4 & 2     & 3     & 3     & \textcolor[rgb]{ .133,  .133,  .133}{$-400<x_n<400$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} &  \\
    \midrule
    33    & ZDT1  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} & \multirow{6}[12]{*}{\cite{RefWorks:271}} \\
\cmidrule{1-7}    34    & ZDT2  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} &  \\
\cmidrule{1-7}    35    & ZDT6  & 2     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<100$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.01$} &  \\
\cmidrule{1-7}    36    & ZDT1  & 3     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
\cmidrule{1-7}    37    & ZDT2  & 3     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
\cmidrule{1-7}    38    & ZDT6  & 3     & 2     & 0     & \textcolor[rgb]{ .133,  .133,  .133}{$0<x_n<50$} & \textcolor[rgb]{ .133,  .133,  .133}{$DI(x_n) = 0.05$} &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:DMOO/Benchmark_Functions2}%
\end{table}%

==> Tables/DMOO/Benchmark_Functions_OLD.tex <==
\begin{table*}[]
\caption{Represent the characteristics of the selected benchmark functions.}
%\label{tab:DMOO/Benchmark_Functions}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}DMOO\\ Problems\end{tabular}}} & \textit{\textbf{d}} & \textit{\textbf{m}} & \textit{\textbf{c}} & \textbf{Characteristics}                                                  & \textbf{\begin{tabular}[c]{@{}c@{}}Continuous \\ variable bound\end{tabular}}                                     & \textbf{\begin{tabular}[c]{@{}c@{}}Discrete \\ interval (DI)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Feasible\\ solutions\end{tabular}} & \textbf{Reference} \\ \hline
Binh2                                                                                  & 2                   & 2                   & 2                   & Concave                                                                   & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}5\\ 0\textless{}x\_1\textless{}3\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 150801                                                                & REF1               \\ \hline
C1\_DTLZ1                                                                              & 2                   & 2                   & 1                   & Linear, Multimodal                                                        & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF2               \\ \hline
C1\_DTLZ3                                                                              & 2                   & 2                   & 1                   & \begin{tabular}[c]{@{}c@{}}Concave, Sphere PF,\\ Multimodal\end{tabular}  & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF3               \\ \hline
C2\_DTLZ2                                                                              & 2                   & 3                   & 1                   & Concave, Sphere PF                                                        & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF4               \\ \hline
C3\_DTLZ4                                                                              & 2                   & 3                   & 2                   & Concave, Biased                                                           & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF5               \\ \hline
ConstrEx                                                                               & 2                   & 2                   & 2                   & NAN                                                                       & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}5\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 45591                                                                 & REF6               \\ \hline
Deep Valley                                                                            & 2                   & 2                   & 0                   & Concave                                                                   & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF7               \\ \hline
DTLZ1                                                                                  & 2                   & 3                   & 0                   & Linear, Multimodal                                                        & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF8               \\ \hline
DTLZ2                                                                                  & 2                   & 3                   & 0                   & Concave, Sphere PF                                                        & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF9               \\ \hline
DTLZ3                                                                                  & 2                   & 3                   & 0                   & \begin{tabular}[c]{@{}c@{}}Concave, Sphere PF, \\ Multimodal\end{tabular} & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF10              \\ \hline
DTLZ4                                                                                  & 2                   & 3                   & 0                   & Concave, Biased                                                           & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF11              \\ \hline
DTLZ5                                                                                  & 2                   & 3                   & 0                   & Concave, Degenerate                                                       & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF12              \\ \hline
DTLZ6                                                                                  & 2                   & 3                   & 0                   & \begin{tabular}[c]{@{}c@{}}Concave, Degenerate,\\  Biased\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF13              \\ \hline
Fonseca                                                                                & 2                   & 2                   & 0                   & Convex                                                                    & \begin{tabular}[c]{@{}c@{}}-4\textless{}x\_0\textless{}4\\ -4\textless{}x\_1\textless{}4\end{tabular}             & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 641601                                                                & REF14              \\ \hline
GLT2                                                                                   & 2                   & 2                   & 0                   & \begin{tabular}[c]{@{}c@{}}Nonlinear disconnected, \\ Convex\end{tabular} & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ -1\textless{}x\_1\textless{}1\end{tabular}              & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 20301                                                                 & REF15              \\ \hline
GLT3                                                                                   & 2                   & 2                   & 0                   & \begin{tabular}[c]{@{}c@{}}Nonlinear disconnected, \\ Convex\end{tabular} & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ -1\textless{}x\_1\textless{}1\end{tabular}              & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 20301                                                                 & REF16              \\ \hline
GLT4                                                                                   & 2                   & 2                   & 0                   & \begin{tabular}[c]{@{}c@{}}Nonlinear disconnected,\\  Convex\end{tabular} & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ -1\textless{}x\_1\textless{}1\end{tabular}              & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 20301                                                                 & REF17              \\ \hline
Kursawe                                                                                & 2                   & 2                   & 0                   & Disconnected concave                                                      & \begin{tabular}[c]{@{}c@{}}-5\textless{}x\_0\textless{}5\\ -5\textless{}x\_1\textless{}5\end{tabular}             & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.1\\ DI(x\_1) = 0.1\end{tabular}    & 10201                                                                 & REF18              \\ \hline
MOP1                                                                                   & 2                   & 2                   & 0                   & Convex                                                                    & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF19              \\ \hline
MOP2                                                                                   & 2                   & 2                   & 0                   & Concave                                                                   & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF20              \\ \hline
MOP3                                                                                   & 2                   & 2                   & 0                   & Discontinued                                                              & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF21              \\ \hline
MOP4                                                                                   & 2                   & 2                   & 0                   & Discontinued                                                              & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF22              \\ \hline
MOP5                                                                                   & 2                   & 2                   & 0                   & Discontinued                                                              & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF23              \\ \hline
NMMin                                                                                  & 2                   & 2                   & 0                   & NAN                                                                       & \begin{tabular}[c]{@{}c@{}}-1000\textless{}x\_0\textless{}1000\\ -1000\textless{}x\_1\textless{}1000\end{tabular} & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 10\\ DI(x\_1) = 10\end{tabular}      & 40401                                                                 & REF24              \\ \hline
Srinivas                                                                               & 2                   & 2                   & 2                   & Convex                                                                    & \begin{tabular}[c]{@{}c@{}}-2\textless{}x\_0\textless{}2\\ -2\textless{}x\_1\textless{}2\end{tabular}             & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 160801                                                                & REF25              \\ \hline
Viennet2                                                                               & 2                   & 3                   & 0                   & Concave                                                                   & \begin{tabular}[c]{@{}c@{}}-4\textless{}x\_0\textless{}4\\ -4\textless{}x\_1\textless{}4\end{tabular}             & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 641601                                                                & REF26              \\ \hline
Viennet3                                                                               & 2                   & 3                   & 0                   & Concave                                                                   & \begin{tabular}[c]{@{}c@{}}-3\textless{}x\_0\textless{}3\\ -3\textless{}x\_1\textless{}3\end{tabular}             & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 361201                                                                & REF27              \\ \hline
Viennet4                                                                               & 2                   & 3                   & 3                   & Convex                                                                    & \begin{tabular}[c]{@{}c@{}}-4\textless{}x\_0\textless{}4\\ -4\textless{}x\_1\textless{}4\end{tabular}             & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 641601                                                                & REF28              \\ \hline
ZDT1                                                                                   & 2                   & 2                   & 0                   & Convex                                                                    & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF29              \\ \hline
ZDT2                                                                                   & 2                   & 2                   & 0                   & Concave                                                                   & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF30              \\ \hline
ZDT3                                                                                   & 2                   & 2                   & 0                   & Discontinuous                                                             & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF31              \\ \hline
ZDT4                                                                                   & 2                   & 2                   & 0                   & Convex, Multimodal                                                        & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ -5\textless{}x\_1\textless{}5\end{tabular}              & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 101101                                                                & REF32              \\ \hline
ZDT6                                                                                   & 2                   & 2                   & 0                   & Concave, Multimodal, Biased                                               & \begin{tabular}[c]{@{}c@{}}0\textless{}x\_0\textless{}1\\ 0\textless{}x\_1\textless{}1\end{tabular}               & \begin{tabular}[c]{@{}c@{}}DI(x\_0) = 0.01\\ DI(x\_1) = 0.01\end{tabular}  & 10201                                                                 & REF33              \\ \hline
\end{tabular}
\end{table*}

==> Tables/DMOO/DV_Pairwise.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[htbp]
  \centering
  \caption{The statistical pair-wise analysis of PCAwMC VS MOEA algorithms with respect to performance indicators (HV, Epsilon, IGD+, and Spread) in Deep Valley problem. Three different symbols are used: "$-$" indicates that there is no statistical significance between the algorithms, "$\blacktriangle$" and "$\triangledown$" were used when PCAwMC achieves statistically better or worse results, respectively than the MOEA algorithms.}
\label{tab:DMOO/DV_Pairwise}
    \begin{tabular}{|c|c|c|c|c|}
    \toprule
    PCAwMC      & HV    & Epsilon & IGD+  & Spread \\
    \midrule
    NSGAII & \blacktriangle     & \boldsymbol{-}     & \blacktriangle     & \blacktriangle \\
    (Sig.) &  (0.040) &  (1.000) & (0.005) &  (0.001) \\
    \midrule
    NSGAIII & \blacktriangle     & \blacktriangle     & \blacktriangle     & \blacktriangle \\
    (Sig.) &  (0.001) &  (0.001) & (0.001) &  (0.001) \\
    \midrule
    SPEA2 & \triangledown     & \triangledown     & \boldsymbol{-}     & \blacktriangle \\
    (Sig.) & (0.001) &  (0.008) & (0.087) &  (0.001) \\
    \bottomrule
    \end{tabular}%
\end{table}%


==> Tables/DMOO/Stat_Results.tex <==
\newpage
\newgeometry{left=5mm, right=5mm}
\begin{center}
%\begin{landscape}
\begin{longtable}{|l|l|l|l|l|l|l|l|l|l|}
\caption{Detailed performance results of the used algorithms across the 38 benchmark problems.} \label{tab:DMOO/Stat_Results} \\
\hline \multicolumn{1}{|p{3.3em}|}{Problem \newline{}ID} &
\multicolumn{1}{c|}{\textbf{PI}} & 
\multicolumn{1}{c|}{\textbf{PCAwMC}} & 
\multicolumn{1}{c|}{\textbf{PCAwLHS}} &
\multicolumn{1}{c|}{\textbf{PCASwMC}} &
\multicolumn{1}{c|}{\textbf{PCASwLHS}} &
\multicolumn{1}{c|}{\textbf{NSGAII}} &
\multicolumn{1}{c|}{\textbf{NSGAII.45}} &
\multicolumn{1}{c|}{\textbf{NSGAIII}} &
\multicolumn{1}{c|}{\textbf{SPEA2}} \\ \hline 
\endfirsthead

\multicolumn{10}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{|p{3.3em}|}{Problem \newline{}ID} &
\multicolumn{1}{c|}{\textbf{PI}} & 
\multicolumn{1}{c|}{\textbf{PCAwMC}} & 
\multicolumn{1}{c|}{\textbf{PCAwLHS}} &
\multicolumn{1}{c|}{\textbf{PCASwMC}} &
\multicolumn{1}{c|}{\textbf{PCASwLHS}} &
\multicolumn{1}{c|}{\textbf{NSGAII}} &
\multicolumn{1}{c|}{\textbf{NSGAII.45}} &
\multicolumn{1}{c|}{\textbf{NSGAIII}} &
\multicolumn{1}{c|}{\textbf{SPEA2}} \\ \hline  
\endhead

\hline \multicolumn{10}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

1 & HV& 55.45 & 64.21 & 234.04 & 244.93 & 172.24 & 170.51 & 62.13 & 280.50 \\
1 & Epsilon & 258.31 & 244.60 & 125.46 & 114.21 & 136.50 & 120.04 & 228.05 & 56.83 \\
1 & IGDP  & 261.59 & 254.09 & 83.10 & 70.90 & 152.91 & 154.28 & 265.81 & 41.33 \\
1 & Spread & 54.54 & 44.29 & 279.58 & 276.71 & 202.59 & 203.13 & 83.30 & 139.88 \\
\rowcolor[rgb]{ .851,  .851,  .851}2 & HV& 160.50 & 160.50 & 160.50 & 160.50 & 160.50 & 160.50 & 160.50 & 160.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}2 & Epsilon & 234.68 & 246.69 & 234.63 & 246.01 & 90.51 & 78.49 & 76.50 & 76.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}2 & IGDP  & 232.94 & 246.49 & 232.80 & 249.78 & 90.48 & 78.53 & 76.50 & 76.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}2 & Spread & 75.59 & 80.08 & 81.71 & 84.63 & 272.25 & 244.49 & 194.20 & 251.06 \\
3 & HV& 64.15 & 86.33 & 221.84 & 237.08 & 172.96 & 168.65 & 165.54 & 167.46 \\
3 & Epsilon & 163.73 & 152.70 & 73.24 & 65.03 & 190.19 & 217.66 & 201.36 & 220.10 \\
3 & IGDP  & 164.56 & 151.13 & 81.25 & 73.19 & 185.66 & 219.80 & 184.13 & 224.29 \\
3 & Spread & 249.15 & 241.25 & 208.55 & 196.06 & 91.24 & 84.95 & 192.30 & 20.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}4 & HV& 88.34 & 72.10 & 143.99 & 126.05 & 215.36 & 190.16 & 210.63 & 237.38 \\
\rowcolor[rgb]{ .851,  .851,  .851}4 & Epsilon & 199.73 & 210.14 & 156.94 & 162.51 & 123.99 & 163.59 & 149.78 & 117.34 \\
\rowcolor[rgb]{ .851,  .851,  .851}4 & IGDP  & 195.78 & 190.00 & 131.84 & 130.99 & 139.74 & 174.40 & 172.83 & 148.44 \\
\rowcolor[rgb]{ .851,  .851,  .851}4 & Spread & 196.86 & 193.30 & 226.26 & 237.23 & 111.05 & 114.19 & 176.60 & 28.51 \\
5 & HV& 38.98 & 42.03 & 256.50 & 256.50 & 163.60 & 169.40 & 100.50 & 256.50 \\
5 & Epsilon & 282.21 & 278.79 & 49.00 & 49.00 & 165.55 & 158.04 & 217.75 & 83.66 \\
5 & IGDP  & 281.55 & 279.45 & 65.00 & 65.00 & 160.79 & 147.06 & 220.15 & 65.00 \\
5 & Spread & 100.69 & 116.83 & 131.99 & 133.93 & 280.03 & 277.31 & 20.53 & 222.71 \\
\rowcolor[rgb]{ .851,  .851,  .851}6 & HV& 68.05 & 53.80 & 238.00 & 238.00 & 190.90 & 190.53 & 66.73 & 238.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}6 & Epsilon & 268.09 & 267.96 & 51.50 & 51.50 & 152.59 & 144.46 & 245.10 & 102.80 \\
\rowcolor[rgb]{ .851,  .851,  .851}6 & IGDP  & 252.78 & 251.33 & 93.00 & 93.00 & 118.00 & 105.50 & 277.40 & 93.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}6 & Spread & 198.85 & 202.96 & 222.60 & 248.33 & 146.39 & 135.96 & 31.84 & 97.08 \\
7 & HV& 77.73 & 83.33 & 257.49 & 258.55 & 161.94 & 163.48 & 20.50 & 261.00 \\
7 & Epsilon & 248.65 & 247.81 & 69.66 & 90.31 & 158.45 & 152.76 & 284.85 & 31.50 \\
7 & IGDP  & 243.79 & 237.21 & 64.86 & 61.41 & 157.58 & 159.65 & 300.50 & 59.00 \\
7 & Spread & 182.93 & 164.19 & 273.21 & 275.35 & 100.25 & 92.59 & 174.99 & 20.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}8 & HV& 75.25 & 78.26 & 215.96 & 219.23 & 222.00 & 222.00 & 29.30 & 222.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}8 & Epsilon & 247.50 & 243.74 & 71.24 & 80.60 & 117.80 & 125.60 & 287.53 & 110.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}8 & IGDP  & 241.33 & 239.18 & 103.00 & 100.00 & 100.00 & 100.00 & 300.50 & 100.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}8 & Spread & 186.09 & 165.39 & 271.86 & 275.89 & 88.91 & 87.49 & 184.60 & 23.78 \\
9 & HV& 72.00 & 80.80 & 233.00 & 233.00 & 205.74 & 197.76 & 28.70 & 233.00 \\
9 & Epsilon & 253.04 & 266.85 & 52.00 & 52.00 & 148.21 & 151.11 & 261.61 & 99.18 \\
9 & IGDP  & 258.73 & 257.23 & 98.00 & 98.00 & 100.50 & 108.00 & 265.55 & 98.00 \\
9 & Spread & 77.81 & 82.31 & 189.98 & 194.76 & 236.65 & 222.43 & 40.38 & 239.69 \\
\rowcolor[rgb]{ .851,  .851,  .851}10& HV& 132.93 & 122.03 & 240.99 & 223.03 & 64.01 & 53.31 & 243.00 & 204.71 \\
\rowcolor[rgb]{ .851,  .851,  .851}10& Epsilon & 187.59 & 196.44 & 134.68 & 135.04 & 261.14 & 263.00 & 24.00 & 82.13 \\
\rowcolor[rgb]{ .851,  .851,  .851}10& IGDP  & 128.05 & 136.08 & 51.74 & 57.73 & 246.81 & 266.36 & 261.03 & 136.21 \\
\rowcolor[rgb]{ .851,  .851,  .851}10& Spread & 165.89 & 189.88 & 197.86 & 193.85 & 226.49 & 227.85 & 23.21 & 58.98 \\
11& HV& 158.05 & 191.69 & 187.41 & 150.65 & 164.45 & 212.51 & 37.30 & 181.94 \\
11& Epsilon & 189.80 & 165.04 & 176.45 & 210.74 & 111.19 & 81.51 & 260.83 & 88.45 \\
11& IGDP  & 137.35 & 121.18 & 125.28 & 150.81 & 182.26 & 123.34 & 293.69 & 150.10 \\
11& Spread & 76.15 & 85.39 & 84.81 & 79.60 & 243.13 & 251.06 & 276.26 & 187.60 \\
\rowcolor[rgb]{ .851,  .851,  .851}12& HV& 132.74 & 142.96 & 146.33 & 145.24 & 200.09 & 179.33 & 123.04 & 214.29 \\
\rowcolor[rgb]{ .851,  .851,  .851}12& Epsilon & 186.85 & 172.35 & 172.50 & 171.84 & 123.75 & 140.75 & 214.58 & 101.39 \\
\rowcolor[rgb]{ .851,  .851,  .851}12& IGDP  & 156.50 & 156.50 & 156.50 & 156.50 & 156.50 & 156.50 & 188.50 & 156.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}12& Spread & 108.66 & 90.73 & 96.96 & 93.03 & 259.91 & 269.60 & 113.15 & 251.96 \\
13& HV& 89.13 & 79.78 & 93.51 & 82.58 & 229.46 & 209.00 & 261.14 & 239.41 \\
13& Epsilon & 216.20 & 231.01 & 217.69 & 231.28 & 105.75 & 121.68 & 67.95 & 92.45 \\
13& IGDP  & 157.00 & 157.00 & 157.00 & 157.00 & 157.00 & 157.00 & 185.00 & 157.00 \\
13& Spread & 102.54 & 132.65 & 114.43 & 128.46 & 272.16 & 276.76 & 26.00 & 231.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}14& HV& 129.69 & 126.50 & 130.13 & 134.83 & 185.48 & 169.36 & 210.85 & 197.18 \\
\rowcolor[rgb]{ .851,  .851,  .851}14& Epsilon & 240.05 & 235.95 & 236.80 & 232.75 & 78.34 & 105.56 & 85.59 & 68.96 \\
\rowcolor[rgb]{ .851,  .851,  .851}14& IGDP  & 160.50 & 160.50 & 160.50 & 160.50 & 160.50 & 160.50 & 160.50 & 160.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}14& Spread & 89.58 & 121.11 & 103.01 & 122.34 & 258.13 & 255.90 & 70.45 & 263.49 \\
15& HV& 90.50 & 84.33 & 77.58 & 91.39 & 227.79 & 228.38 & 241.78 & 242.28 \\
15& Epsilon & 218.59 & 231.81 & 239.18 & 220.10 & 90.68 & 92.84 & 120.84 & 69.98 \\
15& IGDP  & 157.50 & 157.50 & 157.50 & 157.50 & 157.50 & 157.50 & 181.50 & 157.50 \\
15& Spread & 114.99 & 103.04 & 122.13 & 111.25 & 263.00 & 262.88 & 51.10 & 255.63 \\
\rowcolor[rgb]{ .851,  .851,  .851}16& HV& 58.25 & 54.63 & 221.70 & 221.15 & 179.50 & 177.88 & 73.14 & 297.76 \\
\rowcolor[rgb]{ .851,  .851,  .851}16& Epsilon & 242.55 & 254.21 & 151.85 & 149.69 & 141.00 & 130.78 & 186.30 & 27.63 \\
\rowcolor[rgb]{ .851,  .851,  .851}16& IGDP  & 263.35 & 258.44 & 81.64 & 81.59 & 145.45 & 152.26 & 251.19 & 50.09 \\
\rowcolor[rgb]{ .851,  .851,  .851}16& Spread & 143.30 & 141.69 & 251.53 & 246.24 & 208.66 & 210.79 & 22.68 & 59.13 \\
17& HV& 70.11 & 73.91 & 224.00 & 220.73 & 170.99 & 171.11 & 60.75 & 292.40 \\
17& Epsilon & 223.05 & 217.45 & 138.10 & 136.08 & 152.71 & 151.33 & 233.36 & 31.93 \\
17& IGDP  & 208.65 & 213.10 & 74.31 & 76.84 & 184.70 & 152.68 & 277.81 & 95.91 \\
17& Spread & 147.13 & 134.44 & 237.21 & 227.75 & 234.44 & 221.84 & 53.50 & 27.70 \\
\rowcolor[rgb]{ .851,  .851,  .851}18& HV& 68.33 & 64.88 & 239.78 & 249.25 & 161.75 & 164.50 & 54.63 & 280.90 \\
\rowcolor[rgb]{ .851,  .851,  .851}18& Epsilon & 255.43 & 258.93 & 101.36 & 86.68 & 139.21 & 127.64 & 242.23 & 72.54 \\
\rowcolor[rgb]{ .851,  .851,  .851}18& IGDP  & 256.74 & 256.30 & 77.33 & 70.79 & 158.09 & 159.28 & 262.64 & 42.85 \\
\rowcolor[rgb]{ .851,  .851,  .851}18& Spread & 167.15 & 163.43 & 192.59 & 163.60 & 260.30 & 253.63 & 59.26 & 24.05 \\
19& HV& 51.55 & 54.69 & 237.34 & 256.94 & 171.06 & 167.44 & 84.29 & 260.70 \\
19& Epsilon & 264.84 & 258.63 & 78.58 & 59.90 & 146.65 & 158.54 & 249.41 & 67.46 \\
19& IGDP  & 215.91 & 202.04 & 83.06 & 70.50 & 153.64 & 153.64 & 280.28 & 124.94 \\
19& Spread & 80.03 & 82.68 & 283.43 & 273.16 & 194.16 & 204.66 & 20.80 & 145.09 \\
\rowcolor[rgb]{ .851,  .851,  .851}20& HV& 44.71 & 45.53 & 214.05 & 220.10 & 186.74 & 179.45 & 94.75 & 298.68 \\
\rowcolor[rgb]{ .851,  .851,  .851}20& Epsilon & 268.95 & 269.09 & 147.79 & 140.54 & 106.15 & 112.26 & 203.29 & 35.94 \\
\rowcolor[rgb]{ .851,  .851,  .851}20& IGDP  & 249.50 & 252.84 & 93.53 & 91.85 & 138.73 & 148.60 & 279.06 & 29.90 \\
\rowcolor[rgb]{ .851,  .851,  .851}20& Spread & 196.33 & 187.51 & 253.89 & 238.65 & 160.33 & 166.30 & 26.59 & 54.41 \\
21& HV& 48.13 & 45.68 & 186.09 & 198.60 & 202.46 & 189.00 & 119.85 & 294.20 \\
21& Epsilon & 264.78 & 262.58 & 146.10 & 126.33 & 123.73 & 146.51 & 165.89 & 48.10 \\
21& IGDP  & 250.00 & 262.00 & 138.00 & 126.00 & 126.00 & 126.00 & 130.00 & 126.00 \\
21& Spread & 191.51 & 196.54 & 253.61 & 259.41 & 131.96 & 128.45 & 20.55 & 101.96 \\
\rowcolor[rgb]{ .851,  .851,  .851}22& HV& 141.01 & 141.15 & 139.84 & 155.44 & 165.91 & 168.18 & 86.94 & 285.54 \\
\rowcolor[rgb]{ .851,  .851,  .851}22& Epsilon & 136.98 & 133.08 & 213.46 & 191.19 & 183.90 & 157.73 & 197.49 & 70.19 \\
\rowcolor[rgb]{ .851,  .851,  .851}22& IGDP  & 141.31 & 152.56 & 137.88 & 137.88 & 143.56 & 139.38 & 275.31 & 156.13 \\
\rowcolor[rgb]{ .851,  .851,  .851}22& Spread & 206.63 & 198.30 & 279.10 & 270.10 & 111.85 & 109.43 & 20.50 & 88.10 \\
23& HV& 164.33 & 172.98 & 142.59 & 126.90 & 140.56 & 173.68 & 76.55 & 286.43 \\
23& Epsilon & 214.24 & 224.39 & 142.74 & 150.90 & 152.00 & 128.51 & 206.14 & 65.09 \\
23& IGDP  & 179.50 & 183.50 & 159.50 & 171.50 & 187.50 & 171.50 & 187.50 & 43.50 \\
23& Spread & 148.20 & 144.53 & 282.58 & 276.14 & 158.28 & 152.43 & 20.81 & 101.05 \\
\rowcolor[rgb]{ .851,  .851,  .851}24& HV& 67.00 & 64.18 & 160.43 & 196.38 & 182.11 & 178.48 & 152.21 & 283.23 \\
\rowcolor[rgb]{ .851,  .851,  .851}24& Epsilon & 252.13 & 245.70 & 172.80 & 141.91 & 137.54 & 132.54 & 162.10 & 39.29 \\
\rowcolor[rgb]{ .851,  .851,  .851}24& IGDP  & 143.00 & 143.00 & 143.00 & 143.00 & 150.95 & 158.90 & 239.28 & 162.88 \\
\rowcolor[rgb]{ .851,  .851,  .851}24& Spread & 194.64 & 200.16 & 281.00 & 278.08 & 116.60 & 121.60 & 20.50 & 71.43 \\
25& HV& 60.10 & 65.80 & 195.24 & 211.33 & 157.88 & 154.63 & 142.40 & 296.64 \\
25& Epsilon & 235.99 & 248.60 & 145.31 & 150.84 & 122.53 & 148.60 & 196.66 & 35.48 \\
25& IGDP  & 216.25 & 218.28 & 130.00 & 122.50 & 141.25 & 145.00 & 240.73 & 70.00 \\
25& Spread & 193.33 & 175.44 & 286.31 & 256.16 & 132.56 & 132.73 & 20.50 & 86.98 \\
\rowcolor[rgb]{ .851,  .851,  .851}26& HV& 68.05 & 50.26 & 198.70 & 197.33 & 116.44 & 117.95 & 300.25 & 235.03 \\
\rowcolor[rgb]{ .851,  .851,  .851}26& Epsilon & 236.85 & 242.16 & 173.95 & 178.20 & 190.60 & 181.16 & 27.49 & 53.59 \\
\rowcolor[rgb]{ .851,  .851,  .851}26& IGDP  & 205.00 & 217.50 & 57.05 & 58.31 & 197.55 & 181.30 & 87.25 & 280.04 \\
\rowcolor[rgb]{ .851,  .851,  .851}26& Spread & 235.18 & 252.79 & 236.54 & 237.48 & 118.44 & 121.66 & 51.09 & 30.84 \\
27& HV& 74.74 & 89.99 & 144.11 & 142.79 & 131.29 & 150.13 & 251.89 & 299.08 \\
27& Epsilon & 212.11 & 187.96 & 199.74 & 208.28 & 185.74 & 168.54 & 80.04 & 41.60 \\
27& IGDP  & 230.66 & 245.41 & 82.23 & 81.85 & 95.49 & 87.04 & 174.34 & 286.99 \\
27& Spread & 209.08 & 204.58 & 272.76 & 270.26 & 121.54 & 122.91 & 62.38 & 20.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}28& HV& 46.01 & 49.26 & 223.00 & 223.00 & 213.00 & 220.50 & 86.23 & 223.00 \\ 
\rowcolor[rgb]{ .851,  .851,  .851}28& Epsilon & 282.20 & 275.80 & 90.00 & 90.00 & 122.50 & 110.00 & 223.50 & 90.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}28& IGDP  & 273.61 & 268.80 & 100.50 & 100.50 & 100.50 & 100.50 & 239.09 & 100.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}28& Spread & 183.16 & 185.24 & 278.24 & 279.21 & 121.63 & 114.03 & 20.50 & 102.00 \\
29& HV& 138.18 & 144.04 & 280.50 & 280.50 & 129.30 & 121.30 & 20.50 & 169.69 \\
29& Epsilon & 223.46 & 227.59 & 41.64 & 40.24 & 166.34 & 168.48 & 300.50 & 115.76 \\
29& IGDP  & 174.39 & 169.46 & 40.50 & 40.50 & 210.58 & 204.65 & 300.50 & 143.43 \\
29& Spread & 162.25 & 158.54 & 238.91 & 242.05 & 82.31 & 78.89 & 300.50 & 20.55 \\
\rowcolor[rgb]{ .851,  .851,  .851}30& HV& 136.33 & 147.09 & 157.75 & 160.98 & 153.06 & 147.58 & 154.70 & 226.53 \\
\rowcolor[rgb]{ .851,  .851,  .851}30& Epsilon & 182.98 & 212.84 & 199.90 & 198.00 & 123.04 & 121.11 & 181.29 & 64.85 \\
\rowcolor[rgb]{ .851,  .851,  .851}30& IGDP  & 198.68 & 205.18 & 157.49 & 167.15 & 133.06 & 135.44 & 193.84 & 93.18 \\
\rowcolor[rgb]{ .851,  .851,  .851}30& Spread & 70.31 & 85.34 & 88.91 & 83.64 & 247.50 & 251.45 & 186.51 & 270.34 \\
31& HV& 52.15 & 38.79 & 196.60 & 206.00 & 208.90 & 208.93 & 92.28 & 280.36 \\
31& Epsilon & 264.83 & 278.79 & 118.59 & 113.98 & 130.86 & 122.69 & 212.10 & 42.18 \\
31& IGDP  & 268.44 & 279.01 & 80.74 & 67.79 & 148.03 & 146.46 & 223.41 & 70.13 \\
31& Spread & 244.48 & 257.93 & 108.50 & 116.66 & 122.65 & 138.65 & 264.09 & 31.05 \\
\rowcolor[rgb]{ .851,  .851,  .851}32& HV& 46.50 & 65.55 & 182.68 & 186.23 & 177.71 & 171.59 & 173.83 & 279.93 \\
\rowcolor[rgb]{ .851,  .851,  .851}32& Epsilon & 239.93 & 223.05 & 131.46 & 114.71 & 180.04 & 189.69 & 166.90 & 38.23 \\
\rowcolor[rgb]{ .851,  .851,  .851}32& IGDP  & 177.36 & 171.40 & 49.64 & 42.16 & 235.98 & 237.50 & 265.98 & 103.99 \\
\rowcolor[rgb]{ .851,  .851,  .851}32& Spread & 261.39 & 279.18 & 101.96 & 100.58 & 142.29 & 154.34 & 191.56 & 52.71 \\
33& HV& 39.55 & 41.45 & 260.50 & 260.50 & 159.58 & 161.43 & 100.50 & 260.50 \\
33& Epsilon & 281.18 & 279.83 & 40.50 & 40.50 & 161.56 & 159.44 & 220.50 & 100.50 \\
33& IGDP  & 280.38 & 280.63 & 60.50 & 60.50 & 162.45 & 158.55 & 220.50 & 60.50 \\
33& Spread & 229.26 & 228.00 & 250.29 & 252.65 & 120.89 & 121.91 & 60.50 & 20.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}34& HV& 41.03 & 39.98 & 261.00 & 256.51 & 160.33 & 162.68 & 101.49 & 261.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}34& Epsilon & 278.63 & 281.15 & 40.50 & 46.71 & 140.40 & 144.96 & 219.50 & 132.15 \\
\rowcolor[rgb]{ .851,  .851,  .851}34& IGDP  & 281.26 & 279.74 & 60.00 & 64.50 & 160.90 & 158.10 & 219.50 & 60.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}34& Spread & 228.83 & 227.28 & 246.75 & 244.11 & 128.16 & 124.90 & 62.50 & 21.48 \\
35& HV& 37.85 & 43.15 & 220.50 & 220.50 & 220.50 & 220.50 & 100.50 & 220.50 \\
35& Epsilon & 283.36 & 277.64 & 60.50 & 60.50 & 161.61 & 159.39 & 220.50 & 60.50 \\
35& IGDP  & 284.05 & 274.96 & 100.50 & 100.50 & 100.50 & 100.50 & 222.49 & 100.50 \\
35& Spread & 83.96 & 85.86 & 279.28 & 281.45 & 181.85 & 177.10 & 20.50 & 174.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}36& HV& 40.40 & 40.60 & 219.45 & 214.86 & 219.65 & 222.04 & 102.50 & 224.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}36& Epsilon & 281.74 & 279.26 & 47.95 & 53.05 & 141.53 & 135.63 & 215.35 & 129.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}36& IGDP  & 282.06 & 278.94 & 97.74 & 102.45 & 111.90 & 99.91 & 218.50 & 92.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}36& Spread & 227.63 & 201.04 & 257.14 & 236.03 & 121.23 & 114.45 & 20.50 & 106.00 \\
37& HV& 40.71 & 40.29 & 225.50 & 225.50 & 213.06 & 210.94 & 102.50 & 225.50 \\
37& Epsilon & 279.39 & 281.55 & 40.50 & 40.50 & 152.95 & 152.91 & 203.20 & 133.00 \\
37& IGDP  & 280.85 & 280.15 & 40.50 & 40.50 & 146.26 & 147.05 & 217.19 & 131.50 \\
37& Spread & 213.88 & 212.35 & 248.44 & 245.14 & 120.16 & 121.04 & 21.50 & 101.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}38& HV& 41.98 & 39.25 & 217.99 & 217.79 & 221.50 & 221.50 & 102.50 & 221.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}38& Epsilon & 276.20 & 284.45 & 94.33 & 94.48 & 115.43 & 110.13 & 218.50 & 90.50 \\
\rowcolor[rgb]{ .851,  .851,  .851}38& IGDP  & 276.63 & 284.18 & 102.53 & 102.70 & 99.00 & 101.48 & 218.50 & 99.00 \\
\rowcolor[rgb]{ .851,  .851,  .851}38& Spread & 78.96 & 78.96 & 204.45 & 186.60 & 244.65 & 237.23 & 24.15 & 229.00 \\
\end{longtable}
%\end{landscape}
\end{center}
\restoregeometry
\newpage

==> Tables/Model/Experiments_Parameters.tex <==
\begin{table}
  \centering
  \caption{Parameters values for the experiments}
  \label{tab:Model\Experiments_Parameters}
  \begin{tabular}{cccl}
    \toprule
    Parameter&Value&Parameter&Value\\
    \midrule
    $CD$&0.1&$SD$&0.05\\
    $CM$&3000&$PM$&[1,000-10,000]\\
    $CQ$&[0-10]&$PH$&80\\
    $DIFF\_LIMIT$&5&$REP\_LIMIT$&5\\
  \bottomrule
\end{tabular}
\end{table}
